VideoHandles: Editing 3D Object Compositions in Videos Using Video Generative Priors

Generative methods for image and video editing use generative models as priors to perform edits despite incomplete information, such as changing the composition of 3D objects shown in a single image. Recent methods have shown promising composition editing results in the image setting, but in the video setting, editing methods have focused on editing object's appearance and motion, or camera motion, and as a result, methods to edit object composition in videos are still missing. We propose \name as a method for editing 3D object compositions in videos of static scenes with camera motion. Our approach allows editing the 3D position of a 3D object across all frames of a video in a temporally consistent manner. This is achieved by lifting intermediate features of a generative model to a 3D reconstruction that is shared between all frames, editing the reconstruction, and projecting the features on the edited reconstruction back to each frame. To the best of our knowledge, this is the first generative approach to edit object compositions in videos. Our approach is simple and training-free, while outperforming state-of-the-art image editing baselines.

==> Rebuttal/rebuttal_body.tex <==
\makeatletter
\newcommand{\manuallabel}[2]{\def\@currentlabel{#2}\label{#1}}
\makeatother  
\manuallabel{sec:experiments}{5}
\manuallabel{sec:overview}{4}
\manuallabel{sec:warping_function}{4.1}
\manuallabel{eq:3}{3}
\manuallabel{eq:4}{4}
\manuallabel{fig:teaser}{1}
\manuallabel{fig:ablation_study}{6}
\newcommand{\refofpaper}[1]{of the main paper}
\newcommand{\refinpaper}[1]{in the main paper}


% ===== Additional Citation List === %
% [A]: SVD
% [B]: SAM
% [C]: MegaSAM
% [D]: ZeroScope
% [E]: CogVideoX

% ==== Citing Numbers from the main paper === %
% [43]: DUST3R
% [51]: OpenSora
% [28]: Diffusion Handles
% =========================================== %


% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=1.0\linewidth]{Rebuttal/rebuttal_results.pdf}
%     % \caption{}
%     \vspace{-10pt}
%     % \label{fig:rebuttal_teaser}
%     % \vspace{-10pt}
% \end{figure*}

\noindent We thank reviewers for their feedback. We highlight that our method is \emph{``the first attempt to adjust 3D object compositions in videos''} (\RTwo).
We appreciate the reviewers’ recognition of our promising results and training-free approach, which is crucial given the challenge of obtaining paired video data.
%We are happy to see that reviewers appreciate promising results and the training-free nature of our approach, which is crucial in our setting, as gathering paired video data or circumventing the need for it is far from trivial.
%(\ROne, \RTwo)
%Below, we provide a more in-depth response to the reviewers' comments.

\noindent [\ROne, \RTwo] \textbf{Video quality and other video models.}
\hl{Please note that the blurriness in the output is due \emph{not} to our method but to the video generative model we used}, OpenSora~\MyCite{51}.
%: input videos, which are direct outputs from the video model, have quality comparable to our edited outputs. 
Results with a recent more advanced model, CogVideoX~\MyCite{C}, produce much sharper and more detailed outputs, as shown in Figure~\ref{fig:rebuttal_teaser}(a). Since videos cannot be included in the rebuttal, we will add the edited video results in the revision. Notably, the results with CogVideoX also demonstrate our method’s applicability to various video generative models.
% Video quality mainly depends on the video model (quality of input and edited videos is comparable). Open-source models like OpenSora~\MyCite{51} still lag significantly behind commercial variants. However, our method is orthogonal to the choice of video models: Figure~\ref{fig:rebuttal_teaser}(a) \hl{shows two examples} that apply our method to the more recent video model, CogVideoX~\MyCite{E}, yielding sharper and more detailed outputs.
%We clarify that the blurry results and visual artifacts are not solely due to our method but are also influenced by the limited priors of publicly available video diffusion models. As shown in the first example of Figure~\ref{fig:rebuttal_teaser}, A stronger video prior that produces higher-quality generated videos leads to significantly sharper edits, effectively mitigating the blurry issue.

\noindent [\ROne, \RThree] \textbf{Real and stylized videos.}
% \paul{extend this to include style transferred if we have results.}
% Please note that real video editing 
\hl{Please note that the results with real videos are included in our submission} (Figures~\ref{fig:teaser}, \ref{fig:ablation_study}, and lines 518–527, with full videos in the supplement). We present additional editing results for real and stylized videos 
% results with real video edits, along with styled video edits,
in Figure~\ref{fig:rebuttal_teaser}(b) and (c).
% Our method is not limited to generated videos. We show real video editing results (Figures~\ref{fig:teaser}, \ref{fig:ablation_study} and lines 518-527, full videos in the supplement). \hl{An additional real video edit is provided} in Figure~\ref{fig:rebuttal_teaser}(b) and \hl{we also show stylized video edits} in (c). Note that none of the scenes in our videos are synthetic, i.e. procedurally or manually generated.
% We first clarify that our method has proven effective in real video editing, as outlined in Section~\ref{sec:experiments}~\refofpaper{} (lines 518-527). Please refer to the supplementary material, which shows transformations of the selected apple and armchair in real captures. Additionally, the second example in the top figure presents real video editing results using our method with another video diffusion model, CogVideoX~\cite{Yang:2024cogvideox}. Both the results~\refinpaper{} and the additional example show that our method is not limited to generated videos or a specific video generative model.

% \paragraph{[\ROne] Generalizability to Style-Transferred Videos.}
% As discussed above, beyond our method's applicability to real videos, we further demonstrate its generalizability to other types of videos like style-transferred videos. Given the lack of access to pre-trained style-transfer video diffusion models, we generate such videos with the style prompt \texttt{``with low-poly game art style''}. As shown in the last example of Figure~\ref{fig:rebuttal_teaser}, our method successfully transforms the object in the style-transferred video.

% \noindent [\ROne, \RTwo, \RThree] \textbf{Static scene limitation and source of point clouds.}
\noindent [\ROne, \RTwo, \RThree] \textbf{Static scene limitation.}
This limitation is mainly due to the 3D reconstruction method we used, DUST3R~\MyCite{43}.
% , which globally registers per-frame depth estimates. 
Recent advances in dynamic scene reconstruction, such as MegaSAM~\MyCite{B}, could potentially enable our method to handle dynamic scenes. 
% A preliminary result using MONST3R is shown in Figure~\ref{fig:rebuttal_teaser}(b), demonstrating our method's robustness with other reconstruction methods. 
However, note that \hl{even for static scene videos, no prior method has attempted to edit object compositions}, highlighting both the challenge of the problem and the novelty of our work.
% This limitation is mainly due to our 3D reconstruction. As described in line 213, we use DUST3R~\MyCite{43}, which globally registers per-frame depth estimates. We will clarify this point. Recent developments in dynamic scene reconstruction like MegaSAM~\MyCite{C} would likely allow extending our method to dynamic scenes.
% Note, however, that even for videos of static scenes, we know of \hl{no prior method that attempts to edit object compositions.} 
%\Juil{Would it be better to highlight this sentence too?}

% \noindent [\ROne] \textbf{Point cloud warping.}
\noindent [\ROne] \textbf{Consistency of warping.}
Please note that we reconstruct a \emph{single} static 3D point cloud registered across all frames to ensure consistent transformations across frames,
% that the transformations in each frame align with those in other frames, 
as outlined in lines 206-210. We then warp \emph{the 2D features} of each frame in a temporally consistent manner by lifting them onto the reconstructed point cloud, as described in Section~\ref{sec:warping_function}. 

% and warp \emph{2D image features} via unprojection and projection onto the reconstructed 3D point cloud.

% As outlined in lines 206-213, we ensure temporal consistency by editing globally registered points in 3D space, where DUST3R~\MyCite{43} both reconstructs and registers the points.
% Eq.~\ref{eq:3} and~\ref{eq:4} describe how we select 3D points corresponding to an object by linking the object's 2D mask to the point cloud, using camera extrinsics obtained from DUST3R. The 2D mask is obtained with SAM~\MyCite{B}.
%, defined within a shared coordinate system across all frames. 
%We warp 2D image features (not 3D point clouds) based on a reconstructed 3D point cloud that is registered across all frames.
%As mentioned above, our method could potentially be extended for dynamic scenes with recent methods reconstructing 3D point clouds with temporal animation.

\noindent [\ROne] \textbf{Point cloud reconstruction.}
We select 3D points corresponding to an object by linking the object's 2D mask to the point cloud, as described in Eq.~\ref{eq:3} and~\ref{eq:4}. 
% Eq.~\ref{eq:3} and~\ref{eq:4} describe how we select 3D points corresponding to an object by linking the object's 2D mask to the point cloud, using camera extrinsics obtained from DUST3R. 
The 2D mask is obtained with SAM~\MyCite{A}. Unlike PnP, DUST3R~\MyCite{43} predicts the extrinsic matrix, avoiding camera motion constraints, and globally aligns per-frame depths for consistent scaling. We will clarify these points.
% Unlike PnP, DUST3R~\MyCite{43} predicts the extrinsic matrix, avoiding restrictions related to camera motion. It also predicts per-frame depth and aligns depth across frames while optimizing the scale. We will clarify these points.

% \paragraph{[\ROne] Clarifications on Method.}
% As outlined in Section~\ref{sec:overview}~\refofpaper{} (lines 206-213), we ensure temporal consistency of transformations by representing the input video in 3D space with a shared coordinate system across all frames. As noted in line 214, we use DUST3R~\cite{Wang:2024DUST3R} to reconstruct a 3D point cloud $\bm{P}_{\text{src}}$ from the input video. Next, as shown in Equations~\ref{eq:3} and~\ref{eq:4}~\refofpaper{}, the target object's point cloud is obtained by projecting $\bm{P}_{\text{src}}$ into 2D space and selecting the projected points that fall within the 2D object mask region of the first frame, $\C{B}_{\text{src}}^{(1)}$. We compute $\C{B}_{\text{src}}^{(1)}$ using SAM~\cite{Kirillov:2023SAM}, and we will include this detail in the revised version while clarifying how our method ensures temporal consistency.

\noindent [\RTwo] \textbf{Other 3D reconstructions.}
Figure~\ref{fig:rebuttal_teaser}(b) shows results using MONST3R~\MyCite{F} instead of DUST3R~\MyCite{43} for 3D reconstruction, demonstrating the robustness of our method with other 3D reconstruction methods.

\noindent [\RTwo] \textbf{Video length and complex camera movement.}
While we used 51-frame (2-second) videos due to GPU memory limits (80GB on the A100 we used), our method can be applied to longer videos if video models can generate them within limited memory, as 3D reconstruction is relatively lightweight. We present additional 102-frame results in Figure~\ref{fig:rebuttal_teaser}(c), obtained by splitting inference across two GPUs. Additionally, the real video editing results in Figure~\ref{fig:rebuttal_teaser}(b) and in our submission feature complex camera movements in real-world scenarios.

% We use 51-frame (2-second) videos. This is a limitation of the video model we use: GPU memory typically limits open-source models to tens of frames (CogVideoX~\MyCite{E}: 48, ZeroScope~\MyCite{D}: 24, SVD~\MyCite{A}: 25).
% The 3D reconstruction is comparatively lightweight.
% %requiring only 4 minutes to process a 102-frame video on an A6000 GPU.
% Video length also limits the extent of camera movement, given realistic camera speeds. For real videos, we show larger camera motion (see supplement). In Figure~\ref{fig:rebuttal_teaser}(c), \hl{we present 102-frame results} that we obtained by splitting inference across two GPUs.

%\paul{One question for Juil: what enabled us to generate 102 frame videos and why did we not use this for the other results? Is the resolution lower? Did you use another GPU with more memory that you usually don't have access to?}, \Juil{We resolved the VRAM issue by splitting a model into two GPUs.} showing that there is no fundamental limitation in our method.
%We also note that the 3D reconstruction with DUST3R~\cite{Wang:2024DUST3R} is lightweight, requiring only 4 minutes to process a 102-frame video on an A6000 GPU.

% \paragraph{[\RTwo, \RThree] Extensibility to Dynamic Scene Editing.}
% \Juil{Emphasize that our work is the first to edit video with 3D understanding.}
% As discussed in Section~\ref{sec:overview}~\refofpaper{}, our method requires static scenes for 3D reconstruction from the input video. However, with recent advancements in 4D reconstruction~\cite{Zhang:2024monst3r}, our approach could potentially be extended to dynamic scenes. We plan to explore dynamic scene editing in future work using our method, the \emph{first attempt} at object composition editing in videos.




% \paragraph{[\RTwo] Robustness of Our Method with Other Video Diffusion Models.}
% To showcase the adaptability of our training-free approach, we provide video editing results using the recent CogVideoX~\cite{Yang:2024cogvideox} in Figure~\ref{fig:rebuttal_teaser}. As illustrated in the first two examples, our approach is seamlessly integrated with other video diffusion models.

% \paragraph{[\RTwo] Applicability to Long Videos and More Complex Camera Trajectories.}
% In the main paper, we conduct experiments on 2-second videos (51 frames) due to VRAM constraints. While 51 frames represent a reasonable length compared to what publicly available video models can generate (CogVideoX~\cite{Yang:2024cogvideox}: 48 frames, ZeroScope~\cite{Zeroscope}: 24 frames, Stable Video Diffusion (SVD)~\cite{Blattmann:2023SVD}: 25 frames, and Show-1~\cite{Zhang:2023show-1}: 29 frames), we also present a 4-second (102 frames) editing result in the final example of Figure~\ref{fig:rebuttal_teaser}, showing that our method is applicable to longer videos with larger camera rotations. We also note that the 3D reconstruction with DUST3R~\cite{Wang:2024DUST3R} is lightweight, requiring only 4 minutes to process a 102-frame video on an A6000 GPU.

\noindent [\ROne] \textbf{Inference time and computation cost.}
As no other method attempts to edit object compositions in videos, we compare ours with the most technically related image editing method, Diffusion Handles (DH)~\MyCite{28}. While DH requires editing each frame individually, our method processes all frames in a single feed-forward pass, reducing the editing time to 6 minutes compared to DH’s 96 minutes for a 51-frame video.
% As we know of no other method that attempts to edit object compositions in videos, we compare with the technically most related image editing method Diffusion Handles (DH)~\MyCite{28}. Whereas DH needs to edit each frame individually, ours edits all frames in one feed-forward pass, giving us a time of 6 min compared to DH's 96 min for 51-frame videos.
% \hl{365}s
% \hl{5,800}s
%Similar to many video models, our method runs on GPUs with 80GB memory.
% With no prior work, either training-free or training-based, addressing object composition editing in videos, we compare our method's inference time with Diffusion Handles~\cite{Pandey:2024DiffusionHandles}, the state-of-the-art for 2D composition editing. Unlike Diffusion Handles, which edits frames individually, our method leverages a video prior to edit all frames together, achieving faster editing with temporal consistency and more realistic results. \Juil{time comparison} Our training-free method runs within an 80GB VRAM GPU, which is a reasonable cost considering the GPU requirements for training video diffusion models~\cite{Blattmann:2023SVD, Zeroscope, OpenSora, Zhang:2023show-1, Yang:2024cogvideox}.

\noindent [\ROne] \textbf{Evaluating Robustness For Each Visual Variation.}
Thank you for the suggestion. We will include an experiment with synthetic videos featuring diverse visual variations in the final revision.
% We agree that evaluating robustness for each visual variation would lead to a more comprehensive analysis, but generating and collecting such controlled videos is practically challenging. We believe that the diverse visual variations mentioned by the reviewer are already addressed in our experiments.

% We agree that independently evaluating each visual variation factor would be beneficial. However, it is practically challenging to generate and collect videos while controlling each visual variation factor. Nevertheless, we believe that the experiments in the paper already encompass the diverse visual variation scenarios mentioned by the reviewer.


